A Dialogue-based Information Extraction System for Medical Insurance Assessment

In the Chinese medical insurance industry, the assessor's role is essential and requires significant efforts to converse with the claimant. This is a highly professional job that involves many parts, such as identifying personal information, collecting related evidence, and making a final insurance report. Due to the coronavirus (COVID-19) pandemic, the previous offline insurance assessment has to be conducted online. However, for the junior assessor often lacking practical experience, it is not easy to quickly handle such a complex online procedure, yet this is important as the insurance company needs to decide how much compensation the claimant should receive based on the assessor's feedback. In order to promote assessors' work efficiency and speed up the overall procedure, in this paper, we propose a dialogue-based information extraction system that integrates advanced NLP technologies for medical insurance assessment. With the assistance of our system, the average time cost of the procedure is reduced from 55 minutes to 35 minutes, and the total human resources cost is saved 30% compared with the previous offline procedure. Until now, the system has already served thousands of online claim cases.

==> application.tex <==
Based on the previous three steps, the system gets filtered keywords extracted from the real-time conversion text, and derived keywords are classified into different pre-defined topics. To help assessor to better do their job, we customize the Intelligent Insurance Assessment System and identify two types of generic applications: keyword display and report filling. We will describe the details of the application in this section.

\textbf{Keyword Display: }
Keyword display aims at extracting and displaying keywords from the real-time conversation text.
% todo

\textbf{Report Filling: }
Report filling aims at suggesting related content when the assessor fills in the insurance report.
% todo

For the insurance assessor, keyword display and report filling can significantly alleviate the workload of remembering all the claimant information during the inquiry procedure. 


==> system_old.tex <==
\begin{figure*}[ht]
 \centering
 % \includegraphics[width=2.9in, height=1.8in]{workflow.pdf}
 \includegraphics[width=1.8\columnwidth]{figs/workflow.pdf}
 \caption{The workflow of dialogue segmentation, keyword extraction (NER and EL) and keyword filtration (Question and Negation Identification).}
 \label{workflow}
\end{figure*}
Recording the key information during the assessment is tedious for insurance assessors, and junior assessors may even forget to record some important information. To increase the efficiency of information collection and reduce the time cost, the Insurance Assessment System provides a keyword-recommendation feature that first displays keywords in the dashboard and then automatically suggests the related content to be filled. Our system involves different technologies like ASR\footnote{The front end of the Insurance Assessment System displays the real-time video and profile of the claimant.}, NER/EL and question/negation identification to increase the insurance assessment's efficiency.

The whole system is a video dialogue system, built by integrating several independent components, as shown in Figure~\ref{flow}. We have customized the application for the insurance assessment system and identified two types of generic needs: Keyword Display (i.e. extracting and displaying keywords from the real-time conversation text) and Filling Suggestion (i.e. recommend related information when the assessor fills in the different part of insurance report). For insurance assessors, displaying keywords and filling suggestion can alleviate the workload of remembering all the claimant information during the inquiry procedure, as the extracted keyword will be suggested when they fill in the online insurance report. 

The overall workflow (including dialogue segmentation, keyword extraction and keyword filtration) is shown in Figure~\ref{workflow}. For better understanding, we will discuss the technical details in the following subsections.

\subsection{Dialogue Segmentation}
Dialogue segmentation aims at detecting the topic of the real-time conversation text. As the insurance assessment procedure is conducted according to the content that needs to be filled in the insurance report, the different parts of the dialogue between the assessor and claimant are focused on different topics. These topics can be seen as questions that the claimant needs to answer, and we use the sentence similarity learning method to map the utterance from assessors into different topics.

We first order the one-to-many mapping relationship between the topic and standard questions that most assessors inquire in the insurance assessment procedure. Since the way of inquiry among assessors are different, and the ASR results are sometimes affected by the outside speech signal, we use the Enhanced-RCNN model~\cite{enhancedrcnn} to calculate the similarity score between the utterance and pre-defined standard questions, and get the topic of current utterance if the score is greater than the threshold (the default value is 0.5) or follow the topic of the previous utterance if the score is less than the threshold.

After the dialogue segmentation, the whole dialogue is segmented into some parts that belong to different topics. The keyword extracted in the next process will be linked with the corresponding topic. In the following subsection, we will introduce the detail of keyword extraction.

\begin{figure}[ht]
 \centering
 \includegraphics[width=1\columnwidth]{figs/ner_model.pdf}
 % \includegraphics[width=3.1in, height=2in]{ner_model.pdf}
 \caption{The token tagging BERT model for NER.}
 \label{ner_model}
\end{figure}

\subsection{Keyword Extraction}
In the insurance assessment scene, the keyword values that need to be displayed contain five types\footnote{Address, Hospital, Disease, Date, and Examination} and are not within a limit number. Therefore, any string fragment of assessor or claimant utterance may become a keyword value and the traditional DST systems with classification models are unable to predict unseen slot values in a pre-defined value list. Here we convert the keyword extraction as a token tagging task and use the BERT-based NER model to solve it.

We pre-annotate the keyword type in the utterance as \texttt{Addr}, \texttt{Hos}, \texttt{Dis}, \texttt{Date}, \texttt{Exam} or \texttt{Other} (non-named entity) and follow the official tutorial in NER. A visual representation is shown in Figure~\ref{ner_model}. For fine-tuning, we feed the final hidden representation for each token into a classification layer over the NER label set, and the predictions are non-autoregressive, and no CRF \cite{devlin2018bert}. After the NER process, we use the EL model \cite{le2018improving} to link the recognized raw entities to the insurance KB and get the initial keyword. 


\begin{table}[]
\setlength{\tabcolsep}{1mm}
\centering
\begin{tabular}{l|ccccc}
\toprule
\textbf{Entity Type}&\textbf{Addr.}&\textbf{Hos.}&\textbf{Dis.}&\textbf{Date.}&\textbf{Exam.}\\
\hline
F1-Score (\%)&89.9&99.6&95.2&79.3&81.1\\
\bottomrule
\end{tabular}
\caption{The performance of keyword extraction on five entity types.}
\label{table:ner_exp}
\end{table}

% \begin{figure*}[htbp]
%       \centering
%       \subfigure[The Multi-task Model]
%       {
%         \begin{minipage}[t]{0.48\linewidth}
%           \centering
%           \includegraphics[width=0.95\columnwidth]{figs/mtl.pdf}
%         \end{minipage}
%       }
%       \subfigure[The Adversarial Multi-Task Model]
%       {
%         \begin{minipage}[t]{0.48\linewidth}
%           \centering
%           \includegraphics[width=0.95\columnwidth]{figs/adv_mtl.pdf}
%         \end{minipage}
%       }
%       \caption{The structure of Question Identification Model.}
%       \label{fig:adv_mtl}
% \end{figure*}

We take the F1-Score as the evaluation metric of NER/EL, and the experimental results are shown in Table \ref{table:ner_exp}. Next, we will introduce the process of keyword filtration.

\subsection{Keyword Filtration}
During the insurance assessment procedure, the assessor will ask the claimants many detailed questions, including residence/work address, medication experience, disease history, and medical insurance.
As a result, many keyword entities extracted by the previous process are from these assessors' question text and actually do not need to be recommended if the claimant's response has a negative semantics.
To increase the accuracy of keyword recommendation and filter the irrelevant information extracted by the previous keyword extraction process, we use a DST-based method for keyword filtration. Our DST-based method contains two main modules: question identification and negation identification. 
The assessor's conversion text will be first fed to the question identification module.
Suppose the text is identified to be a question. 
In that case, the keyword entities extracted from it will be reserved temporarily and only displayed (or recommended) once they are confirmed by the claimant (decided by the negation identification module).

We will describe more details about the question and negation identification modules in the following subsections.

\subsubsection{Question Identification}
Question identification is to determine whether the current utterance belongs to the insurance assessor's inquiry. We convert question identification as a binary-classification task and utilize text classification model to solve the problem.

We utilize the LSTM~\cite{hochreiter1997long}, one of the most popular text classification models, for the base model to implement question identification. In this case, the input 
\begin{math}
  x = \{x_1, x_2, ..., x_T\}
\end{math}

is the text transformed by the ASR module where $x_t$ is the word after segmentation. The output is a label $y$ indicating whether the text is a question or not. Based on our observation, the topic of insurance assessment is diverse, and the accuracy of question identification is highly relevant to the concrete topic (i.e. residence/work address,  medication experience, or disease history). Therefore, training a single model to cover all the topics is actually not the best solution in our scene, and it is necessary to train different question identification models for different topics. However, the total amount of manually labeled data is not large enough to train multiple classifiers for each topic. 

\begin{table}
  \centering
  \begin{tabular}{l|c}
    \toprule
  \textbf{Model}&\textbf{Accuracy (\%)}\\
    \hline
    Single Model&61.2\\
    Multi-task Model&75.1\\
    Adversarial Multi-task Model&\textbf{78.4}\\
  \bottomrule
\end{tabular}
\caption{Test Performance on Question Identification}
\label{tab:adv}
\end{table}

To alleviate this issue, we use the multi-task learning method\cite{zhang2017survey} to optimize one model and apply in multiple topics by different task layers. As shown in Figure~\ref{fig:mtl}, given an input sequence $x^i$ the calculation formula is as follows:
\begin{align}
  v^s = \mathbf {Encoder}^{share}(x^i)\\
  v^p = \mathbf {Encoder}^{i}(x^i)\\
  \hat y = \sigma (\mathbf W [v^s;v^p] + \mathbf b)
\label{f1}
\end{align}
where the $\mathbf {Encoder}^{share}$ and $\mathbf {Encoder}^i$ represent the public encoder for all topics and the specific encoder of topic $i$ respectively, and $v$ denote the sentence representation after the encoder layer.

We get the final representation by concatenating the share and specific representation and use a sigmoid layer to predict the probability. Here, the entire model is trained end-to-end and use binary-entropy as the loss function:
\begin{align}
  loss(\hat y, y) = -\sum_i y_i\log(\hat y_i)
\end{align}

To further improve the performance of the multi-task model, we adopt an adversarial multi-task learning method (shown in Figure~\ref{fig:adv_mtl}) that the make shared encoder more concentrated on common features\cite{liu2017adversarial, yang2020servicegroup}. The difference with the multi-task learning method is that there is a discriminator to predict the source task $\hat t$ based on the encoder layer's output:
\begin{align}
  \hat t = \mathbf {softmax} (\mathbf U v^s + \mathbf b)
\label{f2}
\end{align}
where $\mathbf U \in \mathbb R ^ {d \times K}$, $\mathbf b \in \mathbb R ^ {1 \times K}$ denote learnable parameters, and $K$ is the number of different tasks. The discriminator minimize the cross entropy of prediction $\hat t$ and the true task label $t$, while the generator-shared encoder maxmize it to encode as less specific features as possible. The loss function can be formulated as:
\begin{align}
  loss_{adv}(\hat t, t) = -\sum_i \sum_k^K t_i^k\log(\hat t_i^k)
\label{f3}
\end{align}
% TODO: Modify the content

Experimental results\footnote{Here the single model represents the original LSTM model} on different training methods are shown in Table~\ref{tab:adv}. The results show that the adversarial multi-task model gets the best accuracy and indicate that the adversarial learning method can improve the question identification's performance for particular topics with only a few labeled data.

\subsubsection{Negation Identification}
After question identification, the following claimant utterance after the identified question will be feed to the negation identification module. 
The system dashboard will only display the keyword extracted from the question if the claimant confirms. 
Here we use a BERT-based binary-classification model for negation identification. The input 
is also the text transformed by the ASR module, and the output is the label indicating whether the text has negative semantics or not. 

The ablation study on the necessity of question and negation identification modules will be present in the experiment section.
